NeRF: Neural Radiance Field in 3D Vision: A Comprehensive Review (Updated Post-Gaussian Splatting)

In March 2020, Neural Radiance Field (NeRF) revolutionized Computer Vision, allowing for implicit, neural network-based scene representation and novel view synthesis. NeRF models have found diverse applications in robotics, urban mapping, autonomous navigation, virtual reality/augmented reality, and more. In August 2023, Gaussian Splatting, a direct competitor to the NeRF-based framework, was proposed, gaining tremendous momentum and overtaking NeRF-based research in terms of interest as the dominant framework for novel view synthesis. We present a comprehensive survey of NeRF papers from the past five years (2020-2025). These include papers from the pre-Gaussian Splatting era, where NeRF dominated the field for novel view synthesis and 3D implicit and hybrid representation neural field learning. We also include works from the post-Gaussian Splatting era where NeRF and implicit/hybrid neural fields found more niche applications. Our survey is organized into architecture and application-based taxonomies in the pre-Gaussian Splatting era, as well as a categorization of active research areas for NeRF, neural field, and implicit/hybrid neural representation methods. We provide an introduction to the theory of NeRF and its training via differentiable volume rendering. We also present a benchmark comparison of the performance and speed of classical NeRF, implicit and hybrid neural representation, and neural field models, and an overview of key datasets.

==> figures/table1old.tex <==
\begin{table*}[ht]
\centering
\caption{Comparison of select NeRF models on the synthetic NeRF dataset
\cite{nerf2020_mildenhall}} \label{tab:benchmark}
\scriptsize
\begin{tabularx}{1.02\textwidth}{l|cccccccc}
Method        & Positional Encoding & Representation & PSNR$\uparrow$ (dB) & SSIM$\uparrow$ & LPIPS$\downarrow$ & Training Iteration & Training Time$^{1}$ & Inference Speed$^{2}$ \\ \hline
Baseline NeRF (2020)\cite{nerf2020_mildenhall} & Fourier \cite{nerf2020_mildenhall}                   & Implicit         & 31.01    & 0.947    & 0.081     &100-300k              & $>$12h  & 1        \\ \hline
\multicolumn{9}{c}{Speed Improvement}
\\ \hline
JaxNeRF (2020)\cite{jaxnerf2020github} & Fourier                    & Implicit           & 31.65    & 0.952    & 0.051     &250k              & $>$12h  & $\sim$1.3        \\ \hline
NSVF (2020) \cite{nerf2020_NSVF} & Fourier                   & Hybrid (Learned)             & 31.74    & 0.953    & 0.047     &  100-150k            & - &$\sim$10                  \\ \hline


SNeRG (2021) \cite{2021sNeRG} & Fourier                   & Explicit (Baked)                & 30.38    & 0.950    & 0.050     &  250k            &$>$12h &$\sim$9000                  \\ \hline 

PlenOctree (2021) \cite{nerf2021_plenoctrees} & SH     & Explicit (Baked)       & 31.71    & 0.958    & 0.053     &  2000k            & $>$12h &   $\sim$3000  \\ \hline

FastNeRF (2021) \cite{2021fastNerf} & Fourier   & Explicit (Baked)         & 29.97    & 0.941    & 0.053     &  300k            & $>$12h &   $\sim$4000  \\ \hline

KiloNeRF (2021) \cite{nerf2021_kilonerf} & Fourier                   & Explicit (Baked)        & 31.00   & 0.95    & 0.03     &  600k+150k+1000k  &$>$12h &$\sim$2000      \\ \hline 

Instant-NGP (2022) \cite{nerf2022_ngp} & Hash Table \cite{nerf2022_ngp}  &  Hybrid (Learned)       & 33.18    & -    & -     &  256k            & $\sim$5m & "orders of magnitude"  \\ \hline

Plenoxels (2021) \cite{2021plenoxels} & SH  &  Explicit (Learned)       & 31.71     & 0.958    &  0.049     &  128k    & $\sim$12m & -  \\ \hline

DVGO (2021) \cite{2021plenoxels} & SH  &  Explicit (Learned)       & 31.95-32.80     & 0.957-0.961    &  0.053-0.27     &  128k    & $\sim$20m & ~45x  \\ \hline

TensoRF (2022) \cite{2022tensorf} & Fourier/SH & Explicit/Hybrid (Learned)& 31.56-33.14 & 0.949-0.963 & - & 15K-30K & ~8-25m & $\sim$100\\ \hline

\multicolumn{9}{c}{Quality Improvement}
\\ \hline

mip-NeRF (2021)\cite{2021mipnerf}      & IPE \cite{2021mipnerf}                 & Implicit       & 33.09    & 0.961    & 0.043     & 1000k              & $\sim$3h  &$\sim$1  \\ \hline 
ref-NeRF (2021)\cite{2022refnerf}      & IPE + IDE \cite{2022refnerf}                 & Implicit             & 35.96    & 0.967    & 0.058     & 250k            &  - &$\sim$1  \\ \hline
\multicolumn{9}{c}{Sparse View/Few Shots}
\\ \hline


MVSNeRF (2021)\cite{2021mvsnerf}      & Fourier                 & Hybrid + Pretrained & 27.07    & 0.931    & 0.163    & 10k (*3 views)            &  $\sim$15m* &$\sim$1  \\ \hline

DietNeRF (2021)\cite{2021dietNeRF}      & Fourier                 & Implicit + Pretrained & 23.15    & 0.866    & 0.109    & 200k (*8 views)            &  - &$\sim$1  \\ \hline

DS-NeRF (2021)\cite{2022dsnerf}      & Fourier                 & Implicit & 24.9    & 0.72   & 0.34    & 150-200k (*10 views)            &  - &$\sim$1  \\ \hline
\end{tabularx}
\flushleft
\small
Key speed, sparse-view and quality improvement models focused on small scale scenes trained on the Synthetic NeRF dataset were selected for comparison.

\footnotesize
$^1$Training speed are given as in the respective original papers. These are to be taken with "a grain of salt", as hardware differences and hyper-parameters such as image/voxel resolution greatly affect training time. 
\footnotesize \\
$^2$Inference speeds are given as speedup factor over the baseline NeRF.
\\

\end{table*}

==> figures/timeline.tex <==
\begin{figure*}[t]
  \centering
\startchronology[startyear=2020, stopyear = 2026,height=1ex,width=\hsize,arrow=False, stopdate=False,startdate=False]
\chronoperiode[datestrue=False]{2020}{2024}{}
\chronoperiode[datestrue=False]{2024}{2025}{}
\chronoevent[textstyle=\bf,
datesstyle=\it,datesseparation=/,conversionmonth=True, textwidth=4.5cm]{19/03/2020}{NeRF\cite{nerf2020_mildenhall}}
\chronoevent[textstyle=\bf,
datesstyle=\it,datesseparation=/,conversionmonth=True, textwidth=4.5cm]{24/03/2021}{mip-NeRF\cite{2021mipnerf}}
\chronoevent[textstyle=\bf,
datesstyle=\it,datesseparation=/,conversionmonth=True, textwidth=4.5cm, markdepth = 200]{25/012/2021}{Plenoctree\cite{nerf2021_plenoctrees}}
\chronoevent[textstyle=\bf,
datesstyle=\it,datesseparation=/,conversionmonth=True, textwidth=4.5cm]{8/8/2023}{Gaussian Splatting\cite{2023gaussian_splatting}}
\stopchronology
  \label{fig:timeline}
\end{figure*}

==> ieeebio.tex <==

\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/Gao.jpg}}]{Kyle Gao}
(Graduate Student Member, IEEE) received his Bachelor’s degree in mathematics from the University of Waterloo, Canada in 2016 and his Master’s degree in physics from the University of Victoria, Canada in 2020, respectively. He is currently pursuing his Ph.D. degree in Systems Design Engineering with the Geospatial Sensing and Data Intelligence Group at the University of Waterloo, Canada. His research interests include computer vision and deep learning. He has published papers in the International Journal of Applied Earth Observation and Geoinformation, Geomatica, and IEEE Transactions on Intelligent Transportation Systems.
\end{IEEEbiography}

\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/Yina.jpg}}]{Yina Gao} is currently pursuing her Bachelor's degree in Engineering Science at the University of Toronto. She is a recipient of the Jane Elizabeth Ham Memorial Scholarship and the University of Toronto Scholar Entrance Scholarship (highest amount). Her research interests are computer vision and deep learning.   
\end{IEEEbiography}


\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/hongjie.jpg}}]{Hongjie He}
(Graduate Student Member, IEEE) received the BSc degree in Geomatics from China University of Petroleum, Qingdao in 2016, the MSc degree in Cartography and Geographic Information Systems from Lanzhou University, China in 2019, respectively. He is currently pursuing his Ph.D. degree in Geography specializing in Applied Earth Observations with the Geospatial Sensing and Data Intelligence Group at the University of Waterloo, Canada. His research interests include AI-based algorithms and software tools for information extraction from earth observation images. He has published papers in the International Journal of Applied Earth Observation and Geoinformation, Canadian Journal of Remote Sensing and Geomatica, flagship conferences including IGARSS and ISPRS.
\end{IEEEbiography}


\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/dening.png}}]{Dening Lu}
received his BSc and MSc degrees in Electrical Engineering, both from the Nanjing University of Aeronautics and Astronautics (NUAA), China in 2018 and 2021, respectively. He is currently pursuing his Ph.D. degree in Systems Design Engineering with the Geospatial Sensing and Data Intelligence Group at the University of Waterloo, Canada. His research interests include 3D point cloud processing and deep learning. He has published papers in IEEE Transactions on Instrumentation and Measurement, IEEE Transactions on Intelligent Transportation Systems, and ICCV.
\end{IEEEbiography}

\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/linlinxu.png}}]{Linlin Xu}(Member, IEEE) received the B.Eng. and M.Sc. degrees in geomatics engineering from China University of Geosciences, Beijing, China, in 2007 and 2010, respectively, and the Ph.D. degree in geography from the Department of Geography and Environmental Management, University of Waterloo, Waterloo, ON, Canada, in 2014. He is currently a Research Assistant Professor with the Department of Systems Design Engineering, University of Waterloo. He has published various papers on high-impact remote sensing journals and conferences. His research interests include hyperspectral imaging, synthetic aperture radar and Lidar, machine learning and environmental monitoring.
\end{IEEEbiography}

\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/junli.png }}]{Jonathan Li}(Senior Member, IEEE) received the Ph.D. degree in geomatics engineering from the University of Cape Town, South Africa, in 2000. He is currently a Professor of Geomatics and Systems Design Engineering, University of Waterloo, Canada. He has supervised 120+ Master's and PhD students as well as postdoc fellows to completion and co-authored 490+ publications, 320+ of which were published in refereed journals, including IEEE Transactions on Geoscience and Remote Sensing (TGRS), IEEE Transactions on Intelligent Transportation Systems (TITS), IEEE Journal of Selected Topics in Applied Earth Observations and Remote Sensing (JSTARS), ISPRS-JPRS, RSE and JAG. He has also published papers in flagship conferences in computer vision and AI, including CVPR, AAAI, and IJCAI. He is the Editor-in-Chief of the International Journal of Applied Earth Observation and Geoinformation (JAG) and the Associate Editor of the TGRS, TITS, and Canadian Journal of Remote Sensing. His main research interests include AI-based information extraction from earth observation images and LiDAR point clouds as well as 3D vision and GeoAI. He is a Fellow of both the Canadian Academy of Engineering and the Engineering Institute of Canada.
\end{IEEEbiography}
